Unsupervised Massive MIMO Channel Estimation with Dual-Path Knowledge-Aware Auto-Encoders

In this paper, an unsupervised deep learning framework based on dual-path model-driven variational auto-encoders (VAE) is proposed for angle-of-arrivals (AoAs) and channel estimation in massive MIMO systems. Specifically designed for channel estimation, the proposed VAE differs from the original VAE in two aspects. First, the encoder is a dual-path neural network, where one path uses the received signal to estimate the path gains and path angles, and another uses the correlation matrix of the received signal to estimate AoAs. Second, the decoder has fixed weights that implement the signal propagation model, instead of learnable parameters. This knowledge-aware decoder forces the encoder to output meaningful physical parameters of interests (i.e., path gains, path angles, and AoAs), which cannot be achieved by original VAE. Rigorous analysis is carried out to characterize the multiple global optima and local optima of the estimation problem, which motivates the design of the dual-path encoder. By alternating between the estimation of path gains, path angles and the estimation of AoAs, the encoder is proved to converge. To further improve the convergence performance, a low-complexity procedure is proposed to find good initial points. Numerical results validate theoretical analysis and demonstrate the performance improvements of our proposed framework.

==> ResponseSection/Abstract.tex <==
\section{Response to the Reviewers’ Comments}

We would like to thank the editor and the reviewers for their comments. We have revised the manuscript to clarify and address the various issues that the reviewers pointed out. In the remainder of this document, we responded to the reviewers’ comments and described the corresponding changes made in the manuscript. The reference numbers for the equations, figures, and tables in this document correspond to those in the revised manuscript. The reference numbers for the bibliography in the revised manuscript are indexed by numbers (e.g., Reference [16]), and those for the bibliography in this answer to reviewers are indexed with a number preceded by the letter “R” (e.g., [R1], [R2]). We mark the changes in the revised manuscript by {\color{blue}blue color}.


==> ResponseSection/Editor.tex <==
\section{Response to Editor}
\textbf{Comment 1:} The motivation of the work in general and the use of VAE for regression and for channel with Gaussian noise is not clear. Simulation results need thorough analyses and compassion of the results to related state of the art methods is required.

\textbf{Response:}
{\guo{
We thank the editor for these comments. 

For the motivation and the use of VAE,

For the simulation results, we only analyze the convergence of the proposed model, while for the calculation, it can be still regarded as a black block. Thus, it is hard to make a general performance analysis of the proposed algorithms.
%
Moreover, we add the SOTA unsupervised-based method proposed in Reference [50] as the comparison in section V to assess the overall performance. Our analysis and design are based on the specific signal propagation model which has no open real transmission data for us to make the experiments.
}}


==> ResponseSection/Reviewer1.tex <==
\section{Response to Reviewer 1}
The authors investigate the problem of channel parameters and angle-of-arrivals (AoAs) joint estimation in the massive MIMO system. As a main contribution, the deep learning-based framework proposed in this paper overcomes two major hurdles in in developing unsupervised methods. Specifically,

\begin{enumerate}
    \item For the uninterpretability/unidentifiability of the latent space, the knowledge-aware decoder is designed with the known channel model and a dual path encoder is designed based on the analysis of independence between differences parameters; Moreover, some model-driven deep learning channel estimation solution can be briefly introduced in the Section I "Model-Driven Deep Learning Based Channel Estimation and Feedback for Millimeter-Wave Massive Hybrid MIMO Systems", IEEE JSAC.
    \item For the problems of getting stuck in global/local optima, rigorous analysis of global optima and local optima is performed. Based on the analyses, the problems is alleviated by a two steps training procedure which is well motivated.
    \item The data preprocessing method and loss function are also carefully designed with mathematical derivations, which can be used for reference to other unsupervised learning methods.
\end{enumerate}

To sum up, it is a heuristic approach to combine classical signal models with deep learning.

~\\ \indent 
\textbf{Comment 1:} The authors mainly compare their approach to other (supervised) AE methods. A SOTA unsupervised benchmark (e.g. the work in Reference [50]) would have helped to asses the overall performance, if possible.

\textbf{Response:}

{\guo{
We thank the reviewer for these comments. We add the SOTA unsupervised-based method proposed in Reference [50] as the comparison in section V to assess the overall performance.
}}

~\\ \indent 
\textbf{Comment 2:} Please specify the value of the precision of the pseudo-label $\Delta_\theta$ in Section III-B.

\textbf{Response:}

The precision $\Delta_\theta$ is set to be $0.01^\circ$ in our numerical simulation. We clarified it in the second paragraph of Section V. We thank the reviewer for the attention to detail. 

~\\ \indent 
\textbf{Comment 3:} In Section III-C, I think the subscript of (14) should be `F' as (7) instead of `2' to denote the Frobenius norm.

\textbf{Response:}

Thanks for raising the concern. The AoAs are assumed to be fixed during the $M$ time slots, as stated at the beginning of Section II. Therefore, the AoA vector $\bm{\theta}$ is a $K \times 1$ vector, as defined after Eqn. (2). Hence, we used the 2-norm in Eqn. (14).

~\\ \indent 
\textbf{Comment 4:} In Section V, it says that ‘Training is done separately for each SNR’ which is costly. Is that possible to train only one specific network and then make estimation for all SNR?

\textbf{Response:}

{\guo{
We thank the reviewer for these comments. If we want to train only one specific network and then make estimation for all SNR, we need to make knowledge adaption between different SNR scenarios. We clarify this problem in the Section VI and will study it in the future work .
}}

~\\ \indent 
\textbf{Comment 5:} The authors should keep the same shape of the lines for the same method in different figure, or it may be confusing.

\textbf{Response:}

{\guo{
We have changed the shape of the lines to make the figure clearer. We thank the reviewer for the attention to detail.
}}

~\\ \indent 
\textbf{Comment 6:} The authors should reconsider the thickness and the color of the lines to make the figure clearer?

\textbf{Response:}

{\guo{
We have changed the thickness and the color of the lines to make the figure clearer. We thank the reviewer for the attention to detail.
}}

~\\ \indent 
\textbf{Comment 7:} The analysis works only when the channel of each user has only one propagation path. Is that possible to extend to multi-path scenario? However, this can be seen as a first step.

\textbf{Response:}

{\guo{
We thank the reviewer for these comments. In this work, we aim to verify the analysis and the framework in AoA and channel estimation scenarios. Thus, we choose the typical one propagation path channel. For the multi-path scenario, we clarify this problem in the Section VI and will study it in the future work .
}}

==> ResponseSection/Reviewer2.tex <==
\section{Response to Reviewer 2}
In this work, the authors propose a model based on the VAE method, for constructing a MIMO channel estimation. They integrate human knowledge for designing and provides deep explanations.

Overall, the paper is well-written and easy to follow. The authors use figures and elaborate on the small details which is highly appreciated.

~\\ \indent 
\textbf{Comment 1:} The suggested framework of multi-path encoder, and a fixed, learned knowledge-aware decoder was sort-of suggested in the past (see [1-2]) as well as unsupervised channel learning frameworks which significantly hurts the novelty of this paper. Therefore, this work plays the only role of extending [1-2] to MIMO communications. However, I found the additional contributions of the paper (the rigorous analysis and the initialization phase) as proper contributions.

[1] Caciularu, Avi, and David Burshtein. "Blind channel equalization using variational autoencoders." 2018 IEEE International Conference on Communications Workshops (ICC Workshops). IEEE, 2018.

[2] Caciularu, Avi, and David Burshtein. "Unsupervised linear and nonlinear channel equalization and decoding using variational autoencoders." IEEE Transactions on Cognitive Communications and Networking (2020).

[3] O’Shea, Timothy J., Tamoghna Roy, and Nathan West. "Approximating the void: Learning stochastic channel models from observation with variational generative adversarial networks." 2019 International Conference on Computing, Networking and Communications (ICNC). IEEE, 2019.

[4] Ye, Hao, et al. "Channel agnostic end-to-end learning based communication systems with conditional GAN." 2018 IEEE Globecom Workshops (GC Workshops). IEEE, 2018.

[5] Raj, Vishnu, and Sheetal Kalyani. "Backpropagating through the air: Deep learning at physical layer without channel models." IEEE Communications Letters 22.11 (2018): 2278-2281.


\textbf{Response:}

{\guo{
We thank the reviewer for these comments. 

For the architecture of the proposed model, ours is similar to the reference paper [1-2] mentioned by the reviewer. But according to different scenarios researched by our work, i.e. AoA estimation which will cause local convergence problem, we rigorously analyze the convergence of our proposed model. This analysis method can be seen as a promising way to analyze the local convergence problem and make the unsupervised learning method more \textit{interpretable/identifiable} which is not trivial.

Thus, our proposed method not only extend [1-2] to MIMO communications, but also introduce a promising way to ensure the convergence of the unsupervised learning method in more complexity searching space.
}}


==> ResponseSection/Reviewer3.tex <==
\section{Response to Reviewer 3}
The authors claim to address the topic of unsupervised AoA and channel estimation in massive MIMO. The general idea of using a variational autoencoder in combination with exploitation of the system knowledge sounds interesting. That said, I have great concerns about the theoretical analysis and technical implementation of the paper (see below).

~\\ \indent 
\textbf{Comment 1:} The variational autoencoder is a generative model for density estimation via Bayesian inference. However, the authors misuse the VAE for regression and learn a reconstruction process. This is simply not in accordance with the concept of VAEs. The authors also make false statements in this direction during the paper. In addition, the distribution of the channels in the paper is Gaussian by definition, which eliminates the purpose of density estimation in the first place, and renders the derivations for the loss function (ELBO) useless.

\textbf{Response:}
{\guo{
We thank the reviewer for these comments. 
}}

~\\ \indent 
\textbf{Comment 2:} The presented simulation results are not adequately explained and the comparisons in the Figures 5-7 are incomprehensible (e.g., the comparison to "standard VAE" or "Correlation" remains unclear). In addition, the presented method is not adequately compared to state-of-the-art methods from both AoA (e.g., advanced MUSIC algorithms, Cramer-Rao bound, unsupervised learning approaches) and channel estimation. Also, the estimation performance of path gains and path angles is constant over the SNR, which is not expected and is not explained by the authors. Moreover, the results of the angle estimates are compared in MSE which is not a suitable metric. This is also true for the path gains/angles. Due to missing information (e.g., definition of SNR, assumption for the definition of $p(Y|z_0,z_m)$ in Appendix B), the results are not reproducible.

\textbf{Response:}
{\guo{
We thank the reviewer for these comments. 
}}

~\\ \indent 
\textbf{Comment 3:} The presented network architecture seems very involved with high computational complexity (2x ResNet with both received signal and covariance matrix as inputs, separate networks for each SNR). The computational complexity is not addressed by the authors and might be intractable in real-time systems.

\textbf{Response:}
{\guo{
We thank the reviewer for these comments. 
}}

~\\ \indent 
\textbf{Comment 4:} The quality of the illustrations are very poor, e.g., the contents of Fig. 4 are inaccessible.

\textbf{Response:}
{\guo{
We thank the reviewer for these comments. 
}}

~\\ \indent 
\textbf{Comment 5:} The paper contains many typographical errors.

\textbf{Response:}

{\guo{
We thank the reviewer for these comments. We have proofread our paper and revised the typographical errors.
}}

==> ResponseSection/Reviewer4.tex <==
\section{Response to Reviewer 4}
\textbf{Comment 1:} First of all, motivations of using unsupervised learning for Massive MIMO is very unclear to me. Supervised learning or self-supervised one should be much better. Please clarify.

\textbf{Response:}

{\guo{
We thank the reviewer for these comments. Deep learning based methods are usually \textit{supervised}, namely requiring accurately labeled data samples and can be only trained offline.
%
In practical, it may be impractical and costly to acquire adequate precise true labels for the channel parameters of interests by field measurements which makes it hard to achieve supervised estimation.
In this sense, unsupervised methods may be more desirable and more aligned with traditional methods, which do not require labeled data and are promising to be developed to online training/updating.

We also add this paragraph into our paper as a motivational statement.
}}

~\\ \indent 
\textbf{Comment 2:} Also, the contributions of this work are rather unclear, and thus, those should be better mentioned.

\textbf{Response:}

{\guo{
We thank the reviewer for these comments. The main contributions of our work are as follows:

\begin{itemize}
    \item \textit{To the best of our knowledge}, an unsupervised channel and AoA estimation framework with rigorous analysis is first proposed for massive MIMO in this paper. Our rigorous analysis of global optima and in the regime of large numbers of antennas, analysis of local optima illustrate the searching space of the framework which can be regarded as a guideline of the design of loss function and the network.
    \item By restructuring the standard VAE, the proposed framework overcomes two challenges in unsupervised channel and AoA estimation. It breaks the hurdle of uninterpretable/unidentifiable latent variables by the knowledge-aware decoder, and alleviates the problem of multiple (bad) local optima by the dual-path encoder. It also shows an effectively way for combining wireless channel knowledge with deep learning.
    \item Informed by the analysis, a two-phase training process is proposed. The first phase initializes the network with good initial points, and the second phase trains the dual-path encoder to learn the global optima. 
\end{itemize}

We have revised our contributions in the Section I of the paper and make it clearer.
}}

~\\ \indent 
\textbf{Comment 3:} Please explain the derived results more intuitively for better understanding.

\textbf{Response:}

{\guo{
We thank the reviewer for these comments. We include some key descriptions in the paper to make the derived results more intuitively for better understanding.
}}

~\\ \indent 
\textbf{Comment 4:} Literature review is not enough. For example, some relevant literature is missing:

[A] "Deep learning based channel estimation for massive MIMO systems,” IEEE Wireless Communications Letters, vol. 8, no. 4, pp. 1228–1231, Aug. 2019.

[B] “Deep Learning Based Channel Estimation for MIMO Systems with Received SNR Feedback,” IEEE Access, vol. 8, pp. 121162–121181, Jul. 2020. 

It would be much better to discuss the above references.

\textbf{Response:}

{\guo{
We thank the reviewer for these comments. We have added [A] and [B] as reference of our paper and discuss them in the Section I. Compared with both reference, our paper fall in a small branch of deep learning based method, i.e. unsupervised learning, and we rigorously analyze the convergence of the proposed framework which make our work more interpretable/identifiable.
}}

~\\ \indent 
\textbf{Comment 5:} More simulation results should be added to better and aggregately validate the effectiveness of the proposed method.

\textbf{Response:}

{\guo{
We thank the reviewer for these comments. We add the SOTA unsupervised-based method proposed in Reference [50] as the comparison in section V to better and aggregately validate the effectiveness of the proposed method.
}}

==> ResponseSection/Reviewer5.tex <==
\section{Response to Reviewer 5}
The general problem fits and the contributions may deserve publication in these transactions. However, major revision is necessary.
Furthermore, I suggested multiple minor changes which would increase the quality of the paper. I suggest to include at least some of them. 

Major comments:

\textbf{Comment 1:} The realization of the system has to be explained in a way that allows an easy implementation in order to reproduce the results!

\textbf{Response:}

{\guo{
We thank the reviewer for these comments. We use a typical deep network model called Resnet with 18 layers to build our proposed model. For clearer description, we add the paper “Deep residual learning for image recognition", which first proposed Resnet and described its structure in details, as key reference.
%
Some essential hyperparameters are provided in Section V, such as 'The neural network is trained using the adaptive moment estimation (Adam) algorithm with a fixed learning rate of $10^{-4}$'. 

And we are sure that follow our description and refer to the paper “Deep residual learning for image recognition", our results can be reproduced.
}}

~\\ \indent 
\textbf{Comment 2:} The referring to multiple references in once should be avoided – in this scope, please check the relevance of all references.

\textbf{Response:}

{\guo{
We thank the reviewer for these comments. We check each reference in our paper again and make sure that the references we refer to are relate to our paper. We also revise the way we introduce the reference and avoid refer to multiple references in once.
}}

~\\ \indent 
Minor comments:

\textbf{Comment 3:} The coverage of the description of the system’s implementation is insufficient. The design of NN-based systems involves a bunch of important design questions, e.g., the network topology and the choice of appropriate hyper parameters. However, the authors only give a name of the topology (ResNet-18) without(!!) any reference and justification, why they use this specific structure. They do not provide essential hyperparameters such as learning rate, … This may not seem important for their contributions, but it prevents (or at least makes it very difficult and time-consuming) to reproduce their results.

\textbf{Response:}

{\guo{
We thank the reviewer for these comments. We use a typical deep network model called Resnet with 18 layers to build our proposed model. For clearer description, we add the paper “Deep residual learning for image recognition", which first proposed Resnet and described its structure in details, as key reference. We also add some essential descriptions about why we use Resnet-18 as our backbone in Section III, i.e. 'For the reason that the signal propagation model is a block fading channel whose fading coefficients will vary block by block forming a large searching space, and the estimations may suffer from a local optimal problem that arise from the hurdle of unsupervised learning. Thus, we use residual connection model to build a deep network for getting more insight and extracting deeper channel information'.

Some essential hyperparameters are provided in Section V, such as 'The neural network is trained using the adaptive moment estimation (Adam) algorithm with a fixed learning rate of $10^{-4}$'.
}}

~\\ \indent 
\textbf{Comment 4:} The results only show the MSE but not the full statistics of the estimation error. However, a major part of this paper is the analysis of the stationary points and the local optima. So, e.g., the error variance, the number of “not properly converged runs”, the relative occurrence per local optima or other statistics may provide significant information.

\textbf{Response:}
{\guo{
We thank the reviewer for these comments. 
}}

~\\ \indent 
\textbf{Comment 5:} A complexity analysis is missing which provides an impression of both the computational complexity but also the effort and duration to train the system.

\textbf{Response:}
{\guo{
We thank the reviewer for these comments. 
}}

~\\ \indent 
\textbf{Comment 6:} A general performance analysis (besides the specific analysis of the proposed algorithms in this paper) may be beneficial. This would include more reference algorithms (including other DL-based methods which are mentioned in the references) and could be based on data from real transmission experiments.

\textbf{Response:}

{\guo{
We thank the reviewer for these comments. 
%
In our paper, we only analyze the convergence of the proposed model, while for the calculation, it can be still regarded as a black block. Thus, it is hard to make a general performance analysis of the proposed algorithms
%
We add the SOTA unsupervised-based method proposed in Reference [50] as the comparison in section V to assess the overall performance. Our analysis and design are based on the specific signal propagation model which has no open real transmission data for us to make the experiments.
}}

~\\ \indent 
\textbf{Comment 7:} The authors refer to more than ten references in once (e.g., [19]-[26], [31]-[45], [31-49]), but only refer to a very few of these references individually as well. Generally, every reference must have it’s own significance and deserves clear and individual mentioning. Although, the referring to multiple references might make sense occasionally, it is too often used in this paper, which gives the impression that either not all references are really relevant or that the referencing is somewhat sloppy at this parts. Hence, I strongly suggest to revise this. Please check each references relevance.

\textbf{Response:}

{\guo{
We thank the reviewer for these comments. We check each reference in our paper again and make sure that the references we refer to are relate to our paper. We also revise the way we introduce the reference and individual mention each significant reference.
}}

~\\ \indent 
\textbf{Comment 8:} Please check the notations, which corresponds not always to the proposed notations, e.g.:

- Equation (3): I assume $\bm{z}$ has to be a matrix of $K \times (1+M)$, $\bm{z}_i$   have to be vectors, so please check the notation! (also, please check if the “double transpose” in Eq. (3) makes sense)

- alpha (path gains) and a (array response vector) look very similar and may get mixed up. Maybe a better solution for it can be found to avoid potential confusion.

- Please check the notations in the appendices, e.g., in Eq (51) the Im-operator seems to be bold.


\textbf{Response:}

{\guo{
We thank the reviewer for these comments.
%
Actually, $\bm{z}_i$  have to be a column vector for $i=0, 1, \ldots, M$ which means that $\bm{z}_i^T$ will be a row vector. Thus, $\bm{z} = \left[ \bm{z}_0^T, \bm{z}_1^T, ..., \bm{z}_M^T \right]^T$ will also be a column vector instead of a matrix of $K \times (1+M)$.

%
alpha (path gains) and a (array response vector)

%
We check the notations in the appendices to make sure that all the notations used in the derivation are correct.
}}

==> ResponseSection/Reviewer6.tex <==
\section{Response to Reviewer 6}
Channel estimation based on expert knowledge and VAE is an interesting topic. Obviously, the simulation results are solid. However, the writing in this manuscript is not enough. My comments are as follow:

\textbf{Comment 1:} Although the technical designs are presented detailly, the motivations are lacking, which makes the manuscript hard to read. For example, the abstract introduces the proposed method directly but the readers cannot know why you propose this method and why this method is helpful. Please reorganize the manuscript thoroughly.

\textbf{Response:}

{\guo{
We thank the reviewer for these comments. 

Deep learning based methods are usually \textit{supervised}, namely requiring accurately labeled data samples and can be only trained offline.
%
In practical, it may be impractical and costly to acquire adequate precise true labels for the channel parameters of interests by field measurements which makes it hard to achieve supervised estimation.
In this sense, unsupervised methods may be more desirable and more aligned with traditional methods, which do not require labeled data and are promising to be developed to online training/updating.

Furthermore, there are two major hurdles in developing unsupervised DL methods for channel and AoAs estimation. The first hurdle is the \textit{uninterpretability/unidentifiability of the latent variables/features} learned. Specifically, the low-dimensional latent variables learned by unsupervised methods usually has no physical meaning. Therefore, if we directly applied an unsupervised learning method to the received signals, the output would not be the parameters we want to estimate (i.e., channel gains and AoAs). This is because without the labels, the network can only take the difference between the input (i.e., the received signals) and its reconstruction based on the latent variables as the loss function. Such a loss function also results in the second hurdle of \textit{multiple local optima}. In other words, there may be multiple sets of channel parameters that are local or global optima of the loss function. Without labels, it is hard to know which set of channel parameters is correct.

In order to further combine deep learning with wireless communication and overcome the above hurdles, we proposed an unsupervised based learning method and make the analysis.

We also reorganize the Section I Introduction and clarify the motivations and contributions separately for clearer description.
}}

~\\ \indent 
\textbf{Comment 2:} This work solves the problems in unsupervised learning. The authors should give a typical scenario, where the supervised learning is useless. For example, if the network is trained offline, the labelled channels are not a problem because the time cost for channel collection is unlimited.

\textbf{Response:}

{\guo{
We thank the reviewer for these comments. 

In practical, it may be impractical and costly to acquire adequate precise true labels for the channel parameters of interests by field measurements which makes it hard to achieve supervised estimation.
In this sense, unsupervised methods may be more desirable and more aligned with traditional methods, which do not require labeled data and are promising to be developed to online training/updating.
}}

~\\ \indent 
\textbf{Comment 3:} Because VAE is widely used in machine learning, the introduction of VAE should be shortened. Please discuss the benefit of applying VAE to channel estimation.

\textbf{Response:}

{\guo{
We thank the reviewer for these comments. 

For the channel parameters estimation, maximum likelihood (ML) will be an optimal criterion for us to design the loss function. However, the posterior probability density functions of the parameters to be estimated are usually unknown and even intractable.
In statistics, it can be solved via variational inference which is widely used in machine learning and can achieve efficiently and reliably approximation. Thus, a promising approach is to approximate ML by variational inference via a variational auto-encoders (VAEs), which are widely used in the literature of DL for unsupervised and semi-supervised learning and have been proven to be effective architectures used in channel estimation
}}

~\\ \indent 
\textbf{Comment 4:} The resolution of figures is low and the characters are small. The legend in Fig. 5(a) is casual. Do ‘MUSIC-’ and ’Music-’ have the same meaning?

\textbf{Response:}

{\guo{
We thank the reviewer for these comments. We have revised the legend Fig. 5(a). We also check other legends in all figure for consistency in our paper.
}}

~\\ \indent 
\textbf{Comment 5:} There are still some typos, such as “simulations validate the theoretical analysis” in conclusion.

\textbf{Response:}

{\guo{
We thank the reviewer for these comments. We have revised the typos pointed out by reviewer. And, we also proofread our paper in case of other typos appear.
}}

~\\ \indent 
\textbf{Comment 6:} The authors have already reviewed on many references but some of them are not close to the proposed method. There some relative studies are ignored. For VAE-based channel estimation, “Domain Knowledge aided Neural Network for Wireless Channel Estimation”. For dual path-based channel estimation, "Dual CNN-Based Channel Estimation for MIMO-OFDM Systems".

\textbf{Response:}

{\guo{
We thank the reviewer for these comments. We add both paper informed by reviewer as key reference in Section I and Section III of our paper when describe our proposed model. Furthermore, we proofread out paper and remove some of the references which are not close to the proposed method.
}}

==> ResponseSection/Reviewer7.tex <==
\section{Response to Reviewer 7}
The authors proposed an unsupervised deep learning-based channel and angle-of-arrivals estimation framework in massive MIMO which estimates the channel efficiently. Overall, the organizational structure of this manuscript is complete, and the proposed method has satisfactory performance.

But there are still some parts of this manuscript needs minor modifications for the improvement:


\textbf{Comment 1:} Introducing the deep learning model for channel estimation is very interesting, but the authors did not show the structure of proposed model and describe it clearly in Section III. Please present the model in detail. The Introduction is good in terms of background. Moreover, contributions of this manuscript are suggested to be placed in the section II, rather than in introduction.

\textbf{Response:}

{\guo{
We thank the reviewer for these comments. We use a typical deep network model Resnet with 18 layers to build our proposed model. For clearer description, we have added the paper “Deep residual learning for image recognition", which first proposed Resnet and described its structure in details, as key reference.

For the Introduction, we reorganize the structure of the Section I and make the motivations and contributions more clearer.
}}

~\\ \indent 
\textbf{Comment 2:} Some key contributions of this approach mentioned should mainly include the highlights compared with the existing results, rather than enumerate the abstract again.

\textbf{Response:}
{\guo{
We thank the reviewer for these comments. 
}}


==> Section/Implementation_Details.tex <==
\section{Implementation Details} \label{sec: Implementation Details}
Before training the network, the sectorization method and the codebook-based correlation are used as data preprocessing and to generate the pseudo-labels, respectively. After sectorization, the range of AoAs estimation is limited so that there is no multi global optima point in the same sector.

During both initialization process and normal training process, the proposed network are trained by adaptive moment estimation (Adam) with learning rate fixed to {$1 \times 10^{-4}$} for weigh updating. The encoder of the network is divided into the channel ResNet and AoA ResNet as a dual path network. Both ResNets in the encoder are implemented by ResNet-18 and the batch size of the input data is set to {$128$}. The input of the channel ResNet is the cascade of the real and imaginary parts of the received signals matrix i.e. {$ \left[ \bm{Y}^R, \bm{Y}^I \right]$}, whose dimension is {$\left( batch size \times 1 \times N_t \times 2M \right)$}. While the AoA ResNet uses the self-correlation matrix as input, i.e. {$ \left[ \bm{R}_{\bm{Y}\bm{Y}}^R, \bm{R}_{\bm{Y}\bm{Y}}^I \right]$} whose dimension is {$\left( batch size \times 1 \times N_t \times 2 N_t \right)$}. The training process of the proposed model is divided into two steps, the initialization and the normal training. The pseudo-labels are only used during initialization of the model. The proposed model uses a training set of {$40000$} samples and a test set of {$10000$} samples generated from the known signal propagation model as \eqref{eqn: AWGN model}.

{\textbf{Initialization Process.}} During this process, loss function \eqref{eqn: Initialization Loss} is used to update the parameters of both ResNets in encoder by back propagation. The pseudo-labels are used to guide the convergence of the AoA ResNet in this step. The maximum epoch of this step is set to {$200$}.

{\textbf{Normal Training Process.}} This process will begin after the model is initialized. \eqref{eqn: Training Loss Function} is used as the loss function during the normal training process. In this step, the proposed model is updated based on totally unsupervised learning. The maximum epoch of this step is set to {$800$}.

==> Section/Related_Work.tex <==
\section{Related Works} \label{sec:related}

{\color{red}
\begin{itemize}
    \item supervised or unsupervised
    \item grid or gridless
    \item technique (e.g., feedforward NN, CNN, convex programming, eigen-decomposition)
\end{itemize}
}

\begin{table*}
\renewcommand{\arraystretch}{1.3}
\caption{Comparison with representative related works}
\label{table:comparison_related_work}
\centering
\begin{tabular}{c|c|c|c|c}
\hline
& \bfseries training & \bfseries unsupervised & \bfseries technique & \bfseries gridless\\
\hline
MUSIC & no & yes & eigendecomposition & no \\
\cite{wang2019super} & no & yes & optimization & yes \\
\cite{liu2018direction} & yes & no & deep learning & no \\
\cite{izacard2019data} & yes & no & deep learning & yes \\
\cite{wu2019deep} & yes & no & deep learning & no \\
\cite{elbir2020deepmusic} & yes & no & deep learning & no \\
proposed & yes & yes & deep learning & yes \\
\hline
\end{tabular}
\end{table*}


\subsection{Classic Signal Processing Algorithms}

MUSIC, ESPIRIT

\cite{barthelme2021doa} used deep learning to reconstruct the covariance matrix and then applied MUSIC.

\cite{elbir2020deepmusic} used deep learning to estimate the MUSIC spectra.

\subsection{Compressive Sensing}

\cite{yang2015enhancing, yang2016exact, chao2017semidefinite, wagner2021gridless, chen2020new}

\cite{wang2019super} formulated the problem as semidefinite programming but used the alternating direction method of
multipliers (ADMM) to achieve lower computational complexity

\cite{yang2021neural} used neural networks to solve the compressive sensing problem. (this is very related to the ICC paper)

\cite{yuan2021unsupervised} used neural networks to solve an optimization problem.

\cite{xu2015active} transforms the problem of active user detection
(AUD) and channel estimation (CE) into standard CS problems and proposes a modified Bayesian CS to conduct AUD and CE in CRAN.

\cite{ke2020compressive} proposes an efficient generalized multiple measurement vector approximate message passing (GMMV-AMP) algorithm to realize
joint AUD and CE based on a spatial domain or an angular domain channel model. Also, a Turbo-GMMV-AMP algorithm is developed for enhanced performance.

\cite{garcia2015low} exploits the use of a large number of antennas at the BSs and the structure and sparsity of the spatial modulation (SM) transmitted signals to improve the performance of conventional detection algorithms based on CS.

\cite{park2018spatial} developed covariance estimation algorithms that are featured by two key ideas, applying the time-varying sensing matrix and exploiting the Hermitian property of the covariance matrix, to achieve spatial channel covariance estimation.

\cite{gao2016structured} proposes a structured compressive sensing (SCS)-based spatio-temporal joint channel estimation scheme with low cost of pilot overhead.

\cite{peng2015an} proposes a presentation of antenna array withvirtual elements (AAVE) by appending additional virtual antenna elements into the original antenna array to achieve fast and high resolution AoA/AoD estimation.

\cite{heath2016an} reduces the training overhead required for accurate channel estimation via CS-based estimation by exploiting the sparsity of mmWave channels.
Similarly \cite{zhou2017low} proposes a CANDECOMP/PARAFAC (CP) decomposition-based method for channel parameter estimation (including angles of arrival/departure, time delays, and fading coefficients).

\cite{gao2018compressive} claims that the mmWave massive MIMO flat-fading channel
estimation can be formulated as the standard CS Model which can be used to estimate AoA.

\subsection{Supervised Deep Learning}

\cite{liu2018direction,su2021mixed, wan2020deep, guo2020doa, akter2021rfdoa, papageorgiou2021deep, barthelme2021machine, pan2021complex}

\cite{izacard2019data}

\cite{wu2019deep}

\cite{pan2021deep} extended \cite{izacard2019data} to 2-D multicomponent sinusoidal signals.

\cite{he2018deep} exploits a learned denoising-based approximate message passing
(LDAMP) network to show the potential of the deep learning method for mmWave channel estimation.

\cite{zhang2020deep} proposes FCDAMP algorithm, combining FCDNet with the LAMP, and obtains high precision of channel estimation and achievable rate by establishing a neural network structure with the better denoising effect.

\subsection{Variational Bayesian Inference}
\cite{badiu2017variational, hansen2018superfast, liu2019super}




